MVS2D: Efficient Multi-view Stereo via Attention-Driven 2D Convolutions

Deep learning has made significant impacts on multi-view stereo systems. State-of-the-art approaches typically involve building a cost volume, followed by multiple 3D convolution operations to recover the input image's pixel-wise depth. While such end-to-end learning of plane-sweeping stereo advances public benchmarks' accuracy, they are typically very slow to compute. We present \ouralg, a highly efficient multi-view stereo algorithm that seamlessly integrates multi-view constraints into single-view networks via an attention mechanism. Since \ouralg only builds on 2D convolutions, it is at least $2\times$ faster than all the notable counterparts. Moreover, our algorithm produces precise depth estimations and 3D reconstructions, achieving state-of-the-art results on challenging benchmarks ScanNet, SUN3D, RGBD, and the classical DTU dataset. our algorithm also out-performs all other algorithms in the setting of inexact camera poses. Our code is released at \url{https://github.com/zhenpeiyang/MVS2D}

==> 06_acknowledgement.tex <==
\paragraph{Acknowledgements.} Qixing Huang would like to acknowledge the support from NSF IIS-2047677 and NSF HDR TRIPODS-1934932. 
